Black-Box Audits for Group Distribution Shifts

When a model informs decisions about people, distribution shifts can create undue disparities. However, it is hard for external entities to check for distribution shift, as the model and its training set are often proprietary. In this paper, we introduce and study a black-box auditing method to detect cases of distribution shift that lead to a performance disparity of the model across demographic groups. By extending techniques used in membership and property inference attacks -- which are designed to expose private information from learned models -- we demonstrate that an external auditor can gain the information needed to identify these distribution shifts solely by querying the model. Our experimental results on real-world datasets show that this approach is effective, achieving 80--100% AUC-ROC in detecting shifts involving the underrepresentation of a demographic group in the training set. Researchers and investigative journalists can use our tools to perform non-collaborative audits of proprietary models and expose cases of underrepresentation in the training datasets.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> sections/general_dist_shift.tex <==
%\vspace{0.5cm}
\subsection{Distribution Shift Audits}\label{sec:disteval}
%DS audits are useful when the auditor's goal is to verify that the audited model's training set comes from a fixed, public distribution $\D$.
%\paragraph{Gender recognition.}
%We explore an application of the GDS audit for fairness.
In this section, we consider that a regulatory agency has standardized a normative distribution $\D$ for the prediction task.
Thus, the audited entity must comply and train their models with data from $\D$.
After observing an accuracy disparity between groups in the target model, the auditor applies our audit to check whether the audited entity is compliant.
%If they are not compliant, our audit would allow the auditor to conclude, with a certain confidence, that they did not use $\D$ to sample the training dataset.

These audits test a more general hypothesis than the GDS audits (\cref{sec:eval}), as they test for any type of shift between the model's training distribution and $\D$.
To illustrate this, consider the shift between \texttt{IncBalance} and \texttt{IncMales}. The DS audits exploit any difference between the two distributions to infer whether the audited model was trained on the distribution of \texttt{IncBalance}, whereas the GDS audits focus on differences that relate to an underrepresentation issue.% in the target model trained on \texttt{IncMales}.

\looseness=-1
%All the experiments in this section use the Simple attack model with $n_q=10$ and $n_s=1$.
Our results show that the audits achieve high statistical power, even for moderate-to-small effect sizes.
%in the use cases that we consider
When we vary the target model's learning algorithm, we observe differences in the audit's performance; in \cref{sec:learning_algo}, we identify several properties of the algorithm that may be involved.
%We also evaluate the Simple attack on some of the data and observe similar audit performance.

\looseness=-1
The baseline for comparison is set by a naive audit that queries the audited model with a sample from $\D$ and concludes that the model was trained on $\D$ if the performance is higher than a certain threshold. Since this naive audit does not have information about the audited model's performance in the control setting, the naive audit's AUC-ROC is $50\%$.

\subsubsection{Statistical Power}
In these experiments, we ensure that $\D$ and $\D'$ are two different distributions.
By taking distributions with an evident shift, we introduce a large effect in the \biased setting.
Thus, we would expect the audit to achieve high true positive rates (TPR) in detecting these shifts.

\begin{table*}
%\rowcolors{1}{}{lightgray}
    \centering
    %\captionsetup{justification=centering,margin=1cm}
	\caption{Configurations of the experiments in \cref{sec:distaudit}, and the audits' results.
% 	%All experiments use the Simple attack with $n_s=1$ and $n_q=10$.
The shift column describes the nature of the DS between the $\D$ and $\D'$ distributions. 
The split size indicates the size of the data partitions into target, shadow, and attack sets. The target and shadow models are trained with the same learning algorithm ($A$).
We report the mean accuracy (and standard deviation) of the target model, and attack models in the control and \biased settings under Accuracy. Finally, the last two columns are the AUC-ROC, and the TPR in the 90th percentile of the control scores.}
	\resizebox{0.99\columnwidth}{!}{
		\input{tables/summary_distshift.tex}}
	\label{tab:experiments_distrib}
%}
%\vspace{-0.5cm}
\end{table*}

\cref{tab:experiments_distrib} lists the setup of these experiments and the datasets we used as samples from $\D$ and $\D'$.
On each run, we split the data into partitions of the same size to train and test the target, shadow and attack models.
The train-test split is 50-50 for the gender recognition models and 75-25 for the other models.
The splits are stratified to preserve the label distribution.
%Stratification is especially important for the US Census prediction tasks, as they tend to be skewed towards the negative class.
%In addition, the DS may involve a shift in the label distributions and, by stratifying the splits, we ensure that the shift is preserved.
For the gender recognition task, we train a Convolutional Neural Network (CNN) (see \cref{sec:appendix_arch} for more details) and use data augmentation to generate slightly different images on every training epoch, eliminating visual differences stemming from image processing.
We thereby discourage the attack model from picking up on visual cues to distinguish the datasets.
For the other tasks we use a Gradient Boosting Machine (GBM) with the hyperparameters in \cite{ding2021retiring}.
%We center-cropped the CelebA images to 60\% of their original size and resized the images in both datasets to the same size.
%This ensures that the images from both datasets are cropped similarly.
%In addition, we horizontally flip all the images uniformly at random. In practice, the auditor knows the target model's input size because she has query access to it, and she can always resize and crop the images from $\D$.
In the table, we also show the target model's mean accuracy on the test sets.
%To measure the target model's performance, we use mean accuracy.
%for the gender recognition task but, because of the class imbalance in the US Census datasets, we use the F1-score for the income and public coverage prediction models.
After training the target model on $\D'$ and testing it on $\D$, we observe a drop in performance for all the tasks, which indicates a significant shift between the distributions.

In \cref{tab:experiments_distrib}, we also show the attack model's mean accuracy in the control and \biased settings.
In the control setting, the attack model's guesses are more accurate than random guessing, but the attack's model mean accuracy in the \biased setting is notably higher. As a result, the audit's AUC-ROC is substantially higher than the baseline (50\%).


\subsubsection{Effect Size}\label{sec:disteffectsize}
The high TPRs in the previous section are expected, as the shift between $\D$ and $\D'$ was large.
We now evaluate the audit for smaller shifts.
To simulate a gradually increasing shift, we sample from the original distributions, denoted by $\D_*$ and $\D'_*$, in proportion to $\alpha\in [0, 1]$: $\D' = \D_*,\;\,\text{ and }\;\,\D = \alpha \, \D_*+ (1-\alpha)\, \D'_*$.

\cref{tab:linear_comb_nn} shows the attack model's accuracy for the income prediction task with a DS along states.
The split size is smaller than the one in previous experiments because we need to combine data from both $\D_*$ and $\D'_*$ to construct the sample from $\D$.
We reserve $11,765$ instances from $\D'_*$ to train the target model in the \biased setting and the rest are mixed with $\D_*$ , from which we draw the sets to train the other models.
%For all the models, we divide each of the sets 75-25 into training and testing.
The different split size between this experiment and the previous ones may account for the slight decrease in the attack's accuracy in the control setting at $\alpha = 0$.

%\setlength{\belowcaptionskip}{-20pt}
\begin{wraptable}{r}{0.49\textwidth}
\rowcolors{5}{}{lightgray}
%\vspace{-0.3cm}
\begin{minipage}{0.49\textwidth}
    \centering
	\caption{The attack's mean accuracy (and standard deviation) in the control and \biased settings for a convex combination of \texttt{IncomeCA} and \texttt{IncomeMI}. The audit's AUC and TPR ($P_{90\%}$) follow. $\alpha$ parametrizes the mixture distribution $\D$.}
	\resizebox{\columnwidth}{!}{\input{tables/convex_gbm.tex}}
	\label{tab:linear_comb_nn}
\end{minipage}
%\vspace{-0.4cm}
\end{wraptable}
%\end{wraptable}

The attack model's accuracy in the control setting is higher than 0.5 for all $\alpha$.
As explained in \cref{sec:learning_algo}, the high capacity of GBMs may account for the high accuracy of the attack in the control setting.
We observe that the accuracy in the \biased setting is approximately linear in $\alpha$, but the audit's performance is not.
%, with a Pearson correlation coefficient of $-0.98$ for 30 equidistant points of $\alpha$.
%However, the auditor's performance is not linear over $\alpha$.
For $\alpha=0.52$, the AUC is close to 100\%, and for $\alpha=0.76$, the AUC is still significantly higher than the naive baseline of 50\%.
This shows that the audits achieve high statistical power even for moderate-to-small effect sizes, despite the decrease in attack accuracy.
Moreover, the linearity of the \biased accuracy implies that the auditor can estimate the shift's magnitude simply by measuring the \biased accuracy.

\subsubsection{Learning Algorithm}
\label{sec:learning_algo}
The learning algorithm $A$ used to train the target model has an impact on the audit's performance.
If $A$ yields different models depending on the training sets, it can boost the attack model's accuracy.
Conversely, if $A$ yields similar models for training sets coming from different distributions, it will be less vulnerable to the attack.
We now test different learning algorithms and identify algorithmic properties that play a role in the audit.

The setup of the experiments here is exactly the same as the one in \cref{sec:disteffectsize}, except that we vary $A$.
The learning algorithms that we tested are: a CART Decision Tree (\texttt{dt}) with a maximum depth of five levels;
a Logistic Regressor with L2 regularization and a limited-memory BFGS solver (\texttt{logit});
a Support Vector Machine with an RBF kernel (\texttt{svm});
a Gaussian Na\"ive Bayes (\texttt{nb});
a Random Forest with 50 estimators (\texttt{rf}); a Multi-Layer Perceptron with the Adam optimizer (\texttt{nn}); and the Gradient Boosting Machine (\texttt{gbm}) with the hyperparameters in \cite{ding2021retiring}.
We use the implementations provided by the Sklearn library, and unless otherwise stated, we use their default hyperparameters.

\begin{figure}
\begin{minipage}{0.50\linewidth}
    \centering
    %\vspace{-0.5cm}
	\resizebox{0.99\textwidth}{!}{\includegraphics{plots/convex_combination.pdf}}
    \captionof{figure}{$\Delta$Accuracy is the difference in attack accuracy between the control and \biased settings. $\alpha$ parametrizes the mixture distribution. The error bands are the 95\% confidence intervals.}
    \label{fig:linear_comb}
    %\vspace{0.5cm}
\end{minipage}
\hfill
\begin{minipage}{0.48\linewidth}
%\vspace{-0.5cm}
\rowcolors{5}{}{lightgray}
	\captionof{table}{Effect of training the target model with different learning algorithms on the audit. We report the attack model's mean accuracy (and standard deviation) in the control and \biased settings for the DS across states, followed by the AUC, and the TPR with the 90th percentile threshold.}
	\resizebox{0.99\columnwidth}{!}{
		\input{tables/folktables_summary}
	}
	\label{tab:dos_summary}
\end{minipage}
%\vspace{-0.6cm}
\end{figure}

\cref{tab:dos_summary} shows the results of the income prediction experiment with a shift along states, and \cref{fig:linear_comb} plots the same for various values of $\alpha$.
The attack model's accuracy in the control setting is around 0.5 for all $\alpha$.
Thus, we again observe from the figure that the accuracy in the \biased setting is approximately linear in $\alpha$ for all $A$.
We also see that the accuracy depends heavily on $A$ as well.
In particular, the accuracy is substantially lower for \texttt{nn}, \texttt{logit}, and \texttt{gnb} than the other algorithms.
Yet, \cref{tab:dos_summary} shows that the audit's test has high statistical power even for these algorithms.
This means that the attack model's accuracy is sufficient for a successful DS audit.
However, this is not the case for higher values of $\alpha$.
At $\alpha=0.75$, the auditor is reduced to the baseline with these algorithms.%, but she still achieves an AUC greater than 80\% with the others.



\paragraph{Learning capacity.} The lower performance of the audit when the target model is trained with \texttt{logit} and \texttt{gnb} can be explained by the relatively low capacity of these algorithms.
When we train the target model on \texttt{IncomeCA} and test on \texttt{IncomeMI}, the \texttt{gnb} and \texttt{logit} models have some of the lowest training accuracies while having also the lowest standard deviations (see \cref{tab:convex_results_generr} in \cref{sec:generalization_errors}), supporting the hypothesis that these algorithms are producing similar, simple models for both distributions and, thus, decreasing the accuracy of the attack. In comparison, \texttt{dt}, \texttt{gbm}, and \texttt{rf} seem to train complex models with significant overfitting (see \cref{tab:convex_results_generr}). 
%indicating a low sensitivity of the algorithm to the shift in ID (DoS),

\paragraph{Variance.}
We also highlight the \texttt{nn} row in \cref{tab:dos_summary}, which shows that the \texttt{nn} algorithm results in the highest standard deviation of the attack model's accuracy in the control setting.
%The \texttt{nn} algorithm tends to result in higher mean and standard deviation in the ID (Probe) and Malware experiments as well (see \cref{tab:probe_summary,tab:malware_summary}).
%In addition, the standard deviation in the target model's accuracy is one order of magnitude higher for \texttt{nn} in all the internet security datasets (\cref{sec:generalization_errors}).
%We do not consider this to be a case of overfitting as the generalization error is low. 
A closer look at individual accuracy reveals that the \texttt{nn} failed to converge for a few seeds.
When this happens, the attack model can easily distinguish between the target and shadow models, increasing both the mean and standard deviation of the attack model's accuracy in the control setting.

We also observe high variance of the attack's accuracy in the \biased setting for some algorithms.
An algorithm's sensitivity to small changes in the training set can be a source of the variance.
More sensitive algorithms can hinder the auditor, as the increased variance in the attack's accuracy distributions can potentially reduce the audit's statistical power.

\paragraph{Data characteristics.}
We have also run all the learning algorithms on the income prediction data with an artificial shift along the sex attribute (the results are in \cref{tab:probe_summary} of \cref{sec:learning_sex_attrib}).
Although the audit is overall less effective on these data because the effect is smaller, we observe that \texttt{gnb} and \texttt{gbm} are still the algorithms where the audits achieve worst and best performance. However, the trend is reversed for \texttt{logit} and \texttt{dt}, compared to the results in \cref{tab:dos_summary}.
A look at the models' generalization error (\cref{tab:convex_results_generr_sex} of \cref{sec:generalization_errors}) shows that it is also reversed: now \texttt{dt} does not overfit, but \texttt{logit} does.
Thus, the interplay between the algorithm and the data also plays a role in the audit's success.

%When we compare the Simple and Complex attacks, we observe that the Simple attack model's control variance is higher than the \biased variance (see \cref{sec:attack_type_comparison}).
%The performance of the audits using the two attack types is similar for all the learning algorithms except for \texttt{nb}, on which the Simple attack is reduced to random guessing in the \biased setting.
%We suspect that the low capacity of the Na\"ive Bayes algorithm is again responsible, as the target model has similar accuracy distributions in the two settings.
%As a result, the Simple attack, which only relies on accuracy information, performs poorly, while the Complex attack may be able to extract other signals from individual inputs.

==> tables/convex_comb_52.tex <==
\begin{tabular}{ccccc}
\toprule
\multicolumn{1}{c}{} & \multicolumn{2}{c}{\textbf{Accuracy}} & \multicolumn{2}{c}{}\\\cmidrule{2-3}
                                  $\boldsymbol{A}$ & \textbf{Control} & \textbf{Shifted} & \textbf{AUC} & \textbf{TPR (}$\boldsymbol{P_{90\%}}$\textbf{)} \\
\midrule
   \texttt{\texttt{\texttt{\texttt{\texttt{dt}}}}} &      52.6±9.76\% &    64.02±11.34\% &      77.80\% &                                            48\% \\
  \texttt{\texttt{\texttt{\texttt{\texttt{gbm}}}}} &     57.48±9.88\% &    81.76±10.02\% &      95.58\% &                                            86\% \\
  \texttt{\texttt{\texttt{\texttt{\texttt{gnb}}}}} &     56.46±6.86\% &    60.94±10.50\% &      61.76\% &                                            38\% \\
\texttt{\texttt{\texttt{\texttt{\texttt{logit}}}}} &     53.62±7.41\% &     59.64±9.13\% &      67.14\% &                                            34\% \\
   \texttt{\texttt{\texttt{\texttt{\texttt{nn}}}}} &     51.36±7.41\% &     59.58±9.47\% &      75.60\% &                                            48\% \\
   \texttt{\texttt{\texttt{\texttt{\texttt{rf}}}}} &     52.54±9.99\% &    73.88±10.50\% &      93.16\% &                                            82\% \\
\bottomrule
\end{tabular}

==> tables/convex_gbm.tex <==
\begin{tabular}{ccccc}
\toprule
\multicolumn{1}{c}{} & \multicolumn{2}{c}{\textbf{Attack Accuracy}} & \multicolumn{2}{c}{\textbf{Audit Perf.}}\\\cmidrule(lr){2-3}\cmidrule(lr){4-5}
$\boldsymbol{\alpha}$ & \textbf{Control} & \textbf{Shifted} & \textbf{AUC} & \textbf{TPR (}$\boldsymbol{P_{90\%}}$\textbf{)} \\
\cmidrule(lr){1-5}

                 0.00 &     56.26±8.94\% &      96.8±4.43\% &        100\% &                                           100\% \\
                 0.28 &     57.88±8.91\% &     93.28±6.73\% &      99.94\% &                                           100\% \\
                 0.52 &     57.48±9.88\% &    81.76±10.02\% &      95.58\% &                                            86\% \\
                 0.76 &    60.08±10.93\% &     65.72±9.27\% &      65.82\% &                                            10\% \\
                 1.00 &     59.34±9.00\% &     57.68±9.87\% &      46.80\% &                                             8\% \\
\bottomrule
\end{tabular}

==> tables/summary_distshift.tex <==



\begin{tabular}{cccccccccccc}
\toprule
\multicolumn{6}{c}{\textbf{Experiment Configuration}} & 
\multicolumn{3}{c}{\textbf{Accuracy}} &  \multicolumn{2}{c}{\textbf{Audit Perf.}}\\\cmidrule(lr){1-6}\cmidrule(lr){7-9}\cmidrule(lr){10-11}
                  \textbf{Task}  	&
			\textbf{Shift} &
			$\boldsymbol{\D}$ &  $\boldsymbol{\D'}$	& \textbf{Split Size}  & $\boldsymbol{A}$ &
			\textbf{Target} &
			\textbf{\makecell{Attack  (Control)}}
			 &
			\textbf{\makecell{Attack (Shifted)}}
			  & \textbf{AUC} & \textbf{TPR (}$\boldsymbol{P_{90\%}}$\textbf{)} \\
\cmidrule(lr){1-11}
    \makecell{Gender \\ recog.}	&
			Fame &
			\texttt{CelebA}		  	  & \texttt{UTKFace}			& $\approx{8}$K		 				    & CNN 		    & $93.50\pm 0.83$\% &     51.51±3.82\% &     98.44±1.10\% &        100\% &                                           100\% \\
\addlinespace
Income &
			State &
			\texttt{IncomeCA}   	  	  &  \texttt{IncomeMI}			&  		$\approx37.5$K	 						& GBM 			& $72.64\pm 0.56$\% &   58.78±10.80\% &     100.00±0.00\% &      100\% &       100\% \\
%\addlinespace
prediction &
			 Sex &
			 \texttt{IncBalance}   	  	  &  \texttt{IncMales}			&  		$30$K	 						& GBM 			& $78.82\pm 0.50$\% & 57.66±8.73\% &     75.59±10.02\% &      91\% &                                            68\% \\
\addlinespace
\makecell{Public cov.\\ prediction} & Year
			& \texttt{PubCov18}   	  	  &  \texttt{PubCov14}			&  		35K	 						& GBM 			& $72.90\pm 0.22$\% & $55.56\pm 7.57$\% &     $74.71\pm 9.35$\% &      94\% &                                            86\% \\
\bottomrule
\end{tabular}

